Cooperative Multi-Agent Reinforcement Learning via Epigraph-Form Guided Exploration

Discovering cooperative behavior in multi-agent reinforcement learning (MARL) is challenging due to the combinatorial complexity of joint state-action spaces, which hinders the emergence of coordinated behaviors from trial-and-error alone. Intrinsic rewards are often used to aid discovery, but naively combining them with team objectives can distort the learning signal, compromising task performance. In this paper, we propose EFXPLORER, a constrained exploration framework that maximizes exploration objectives subject to a constraint that preserves established task performance. We solve the resulting problem using an epigraph reformulation that introduces adaptive exploration budgets. This approach separates intrinsic rewards from task objectives and regulates exploration through task feasibility. To further encourage diverse and temporally extended exploration, we incorporate a successor distance-based intrinsic reward that captures long-horizon dependencies. Empirically, our method outperforms strong baselines and induces novel cooperative strategies across SMAX, VMAS, and MPE benchmark suites.

==> macros.tex <==
\makeatletter
\usepackage{kotex}
\usepackage{amsmath}
\DeclareMathOperator*{\argmax}{argmax}

\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}
% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{caption}

\usepackage{hyperref}
% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}
\usepackage[most]{tcolorbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

\usepackage{thm-restate}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{microtype}
\usepackage[dvipsnames]{xcolor}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{tikz-cd}
\usepackage{subcaption}
\usepackage{comment}
% \usepackage[numbers]{natbib}
\usepackage{physics}
\usepackage{tikz-cd}
\usepackage{wrapfig}
\usepackage{tcolorbox}
\usepackage{enumitem}
\usepackage{cancel}
\usepackage{placeins}
\usepackage{bbm}
\usepackage{tikz}
\usepackage{enumitem}
\usepackage[mode=image]{standalone}
\usepackage{pgfplots}
\usepackage{tikz}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.18}
\usepgfplotslibrary{fillbetween}
\usepackage{graphicx}
\usepackage{multirow}
\usetikzlibrary{pgfplots.colorbrewer,calc}

\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{booktabs} % for professional tables

\usepackage{subfiles}
\usepackage{csquotes}
\usepackage[table]{xcolor} 
\usepackage{annotate-equations}
\usepackage[subfigure]{tocloft}
\usepackage{array}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsbsy}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{titlesec}

\captionsetup[algorithm]{labelsep=colon}

\usetikzlibrary{calc,fadings,fit}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{shapes,arrows,backgrounds,positioning}

\let\includegraphics@i\includegraphics
\renewcommand\includegraphics[1][width=\linewidth]{\includegraphics@i[#1]}

% \usepackage{mathcommands}

\theoremstyle{plain}

\let\blacksquare@i\blacksquare
\def\blacksquare{\raisebox{-0.17ex}{$\blacksquare@i$}}

\allowdisplaybreaks
\makeatother

% Colors 
\definecolor{wine}{RGB}{204, 0, 102}
\definecolor{magenta_wine}{RGB}{158, 44, 143}
\definecolor{dusty_wine}{RGB}{143, 59, 101}
\definecolor{ocean}{RGB}{13, 121, 202}
\definecolor{light_ocean}{RGB}{18, 178, 235}
\definecolor{dark_ocean}{RGB}{10, 89, 148}
\definecolor{grey}{RGB}{170, 170, 170}
\definecolor{light-grey}{RGB}{220, 220, 220}
\definecolor{dark_gray}{rgb}{0.2, 0.2, 0.2} 
\definecolor{med-grey}{rgb}{0.3, 0.3, 0.3} 
\definecolor{grape}{RGB}{112,48,160}
\definecolor{aqua}{RGB}{52,172,139}
\definecolor{dark_aqua}{RGB}{35,115,93}
\definecolor{dark_orange}{RGB}{216,92,0}
\definecolor{vibrant_orange}{RGB}{250, 160, 26}
\definecolor{vibrant_blue}{RGB}{14, 120, 255}
\definecolor{vibrant_pink}{RGB}{255, 0, 104}
\definecolor{dark_red}{RGB}{122, 0, 0}
\definecolor{dark_green}{RGB}{0, 92, 34}
\definecolor{dusty_blue}{RGB}{77, 91, 128}
\definecolor{dark_brown}{RGB}{125, 54, 36}
\definecolor{violet}{RGB}{116, 12, 173}

\renewcommand*{\eqnhighlightcolorbox}[2]{%
% \colorbox sets the second argument in text mode, so for use within equations we wrap it in $ $ again
    \mathchoice% to get right font size in each mode:
        {\colorbox{#1}{$\displaystyle #2$}}%
        {\colorbox{#1}{$\textstyle #2$}}%
        {\colorbox{#1}{$\scriptstyle #2$}}%
        {\colorbox{#1}{$\scriptscriptstyle #2$}}%
}

%%% the fbox with 0pt rule fixes the height of eqnmark vs eqnmarkbox issue
\renewcommand*{\eqnhighlightfbox}[2]{%
% \fbox sets the second argument in text mode, so for use within equations we wrap it in $ $ again
    \mathchoice% to get right font size in each mode:
        {\begingroup\setlength{\fboxrule}{0pt}\fbox{$\displaystyle\color{#1}#2$}\endgroup}%
        {\begingroup\setlength{\fboxrule}{0pt}\fbox{$\textstyle\color{#1}#2$}\endgroup}%
        {\begingroup\setlength{\fboxrule}{0pt}\fbox{$\scriptstyle\color{#1}#2$}\endgroup}%
        {\begingroup\setlength{\fboxrule}{0pt}\fbox{$\scriptscriptstyle\color{#1}#2$}\endgroup}%
}

% . is the current color

\renewcommand*{\eqnhighlight}[2]{\begingroup\colorlet{currentcolor}{.}\eqnhighlightcolorbox{#1!\eqnhighlightshade}{\eqnhighlightheight #2}\endgroup}
\renewcommand*{\eqncolor}[2]{\begingroup\colorlet{currentcolor}{.}\eqnhighlightfbox{#1}{\eqnhighlightheight #2}\endgroup}

%%% Arguments to \eqnmark[box]: [highlight color]{node name}{term to highlight}
\renewcommand*{\eqnmarkbox}[3][currentcolor]{\addvalue{#2}{#1}\tikzmarknode{#2}{\eqnhighlight{#1}{#3}}}
\renewcommand*{\eqnmark}[3][currentcolor]{\addvalue{#2}{#1}\tikzmarknode{#2}{\eqncolor{#1}{#3}}}

\makeatletter
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-0.08in}{0.01in}
                {\normalsize\bf\raggedright}}
\makeatother

\usepackage[export]{adjustbox}
